Isotropic SGD: a Practical Approach to Bayesian Posterior Sampling

In this work we define a unified mathematical framework to deepen our understanding of the role of stochastic gradient (SG) noise on the behavior of Markov chain Monte Carlo sampling (SGMCMC) algorithms. Our formulation unlocks the design of a novel, practical approach to posterior sampling, which makes the SG noise isotropic using a fixed learning rate that we determine analytically, and that requires weaker assumptions than existing algorithms. In contrast, the common traits of existing \sgmcmc algorithms is to approximate the isotropy condition either by drowning the gradients in additive noise (annealing the learning rate) or by making restrictive assumptions on the \sg noise covariance and the geometry of the loss landscape. Extensive experimental validations indicate that our proposal is competitive with the state-of-the-art on \sgmcmc, while being much more practical to use.

==> alphaestim.tex <==
 A shared assumption of \sgmcmc methods is the Gaussianity of \sg noise. While this can be justified with the c.l.t  for relatively simple models (linear models or simple feed-forward networks), this assumption has been challenged in the deep learning domain \cite{csimcsekli2019heavy,pmlr-v97-simsekli19a} (see also results in the appendix ) suggesting that from complex architectures the noise distribution is heavy tailed. In particular, the hypothesis is that the noise follows and \tetxtit{$\alpha$-stable} distribution, i.e.
 \begin{equation}
     w\sim p(w)=\mathcal{F}^{-1}\left(\exp(-|ct|^{\alpha})\right)
 \end{equation}
 where $\alpha \in [0,2]$. Notice that except for particular cases, $p(w)$ can not be expressed in closed form.  \giulio{Not sure about (0 or [ 0}
 In general, when $\alpha<2$ the variance of the distribution goes to infinity and thus dealing with all methods that require the estimation or the usage of a covariance is tricky. It is interesting to underline that for $\alpha=2$ the distribution is the usual Gaussian one.

 Having acknowledged that the noise is not Gaussian for deep models (at least) two possibilities can be considered: the first one is to study the \sde with Lèvy Noise instead of Brownian, using a formalism similar to the one considered in \cite{csimvsekli2017fractional}, where \textit{fractional} \fpe have been considered. Several practical difficulties are however tied to this choice, such as the necessity to numerically approximate the fractional derivative of order $\alpha$ or the necessity to have full batch evaluations (in \cite{csimvsekli2017fractional} mini-batches are also considered but the role of implicit noise is neglected). \giulio{I would like to avoid to give away for free this idea, I think this could be an insteresting and unexplored future work.}
 The second possibility, the one we pursued in this work, is to \giulio{neglect the fact that the noise is non-gaussian, treat it as an approximation error and use for the theoretical calculations the gaussian distribution that is closest to the real noise distribution /don't like the sentence}. In particular, for the one dimensional case, we minimize the $l_2$-distance \giulio{I found a sign mistake in the derivation of KL bound, I had to redo the calculations with a different distance. From a practical (and thus experimental) point of view the difference is minor} between $p(x)$ and $q(x)$, where $p(x)=\sqrt{2\pi\sigma^2}\exp\left(-\frac{x^2}{2\sigma^2}\right)$ and $q(x)=\mathcal{F}^{-1}\left(\exp(-|ct|^{\alpha})\right)$. As stated above, in general no closed form exists for $q(x)$. Thanks to Parseval equality, however, we can compute the distance in the frequency domain between the two distributions, i.e.
 \begin{equation}
     C=\int\limits_{-\infty}^{+\infty} |p(x)-q(x)|^2 dx=\int\limits_{-\infty}^{+\infty} |p(t)-q(t)|^2 dt
 \end{equation}
 where $p(t)=\exp(-\frac{\sigma^2 t^2}{2})$ and $q(t)=\exp(-|ct|^{\alpha})$. Since we are optimizing w.r.t. $\sigma$, we can write the equivalent cost function
 \begin{flalign}
     &C_{eq}=\int\limits_{-\infty}^{+\infty} |p(t)|^2 dt-2\int\limits_{-\infty}^{+\infty} p(t)q(t) dt=\int\limits_{-\infty}^{+\infty} \exp(-\sigma^2 t^2)dt -2 \int\limits_{-\infty}^{+\infty} \exp(-\frac{\sigma^2 t^2}{2})\exp(-|ct|^{\alpha})dt\nonumber\\&\frac{\sqrt{\pi}}{\sigma}-\frac{2}{\sigma}\int\limits_{-\infty}^{+\infty} \exp(-\frac{\tau^2}{2})\exp(-|\frac{c}{\sigma}\tau|^{\alpha})d\tau=\frac{\sqrt{\pi}}{\sigma}-\frac{2\sqrt{2\pi}}{\sigma}\int\limits_{-\infty}^{+\infty}\frac{1}{\sqrt{2\pi}} \exp(-\frac{\tau^2}{2})\exp(-|\frac{c}{\sigma}\tau|^{\alpha})d\tau\nonumber=\\&\frac{1}{\sigma}\left(\sqrt{\pi}-\sqrt{2\pi}E_{T\sim N(0,1)}[\exp\left(-|\frac{c}{\sigma}T|^{\alpha}\right)]\right).
 \end{flalign} 
 Equivalently, we can maximize for $r=\frac{c}{\sigma}$, the following function $r\left(\sqrt{\pi}-\sqrt{2\pi}E_{T\sim N(0,1)}[\exp\left(-|rT|^{\alpha}\right)]\right)$. The expected value does not have a closed form solution, but since the integral is single dimensional, it is possible to integrate numerically and derive the optimal $r$ for a given tail index, i.e. $\hat{r}=\arg\min C(r,\alpha)$ and consequently the optimal $\sigma$ as $\hat{\sigma}=\frac{c}{\hat{r}}$  (see figure \ref{fig:rvsalpha}. Notice that even for moderately small values of $\alpha$ (i.e. $\alpha>0.5$), the optimal value is roughly $\frac{1}{2}$ (red line), implying that a matching of the scales is sufficient. In our implementation a simple lookup-table computed once is sufficient to derive the optimal $\sigma$ given knowledge of $\alpha,c$
 \begin{figure}
     \centering
     \includegraphics[scale=0.4]{figures/rvsalpha.jpg}
     \caption{Caption}
     \label{fig:rvsalpha}
 \end{figure}
 The parameters $\alpha,c$ are estimated   ( extending the results  of \cite{vehel2018explicit}to space varying settings  \giulio{? check if peer-reviewed}) as follows
 \begin{flalign}
     11
 \end{flalign}

==> broader.tex <==
The work presented in this article aims at turning sophisticated methods for the accurate quantification of uncertainty associated with statistical models, into practical algorithms. Many application domains, including health-care, life and environmental sciences, to name a few, can benefit from being able to inform decisions based on more than a simple predictive mean. Efficient and practical methods for computing full predictive distributions based on theoretically sound principles are thus of paramount importance, as they enable reasoning about the risks associated to crucial decisions.

The fundamental goal of this work is to benefit machine learning practitioners, because it lowers the effort that is generally required to use, and appropriately tune, \sgmcmc methods. In fact, our method does not require creative and exhausting hyper-parameter tuning, which is both a time and energy consuming endeavor. Our hope is for the method presented in this article to help \sgmcmc algorithms reach a wider audience.


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

